Enabling Low-Overhead Over-the-Air Synchronization Using Online Learning

Accurate network synchronization is a key enabler for services such as coherent transmission, cooperative decoding, and localization in distributed and cell-free networks. Unlike centralized networks, where synchronization is generally needed between a user and a base station, synchronization in distributed networks needs to be maintained between several cooperative devices, which is an inherently challenging task due to hardware imperfections and environmental influences on the clock, such as temperature. As a result, distributed networks have to be frequently synchronized, introducing a significant synchronization overhead. In this paper, we propose an online-LSTM-based model for clock skew and drift compensation, to elongate the period at which synchronization signals are needed, decreasing the synchronization overhead. We conducted comprehensive experimental results to assess the performance of the proposed model. Our measurement-based results show that the proposed model reduces the need for re-synchronization between devices by an order of magnitude, keeping devices synchronized with a precision of at least 10 microseconds with a probability 90%.

==> SotA.tex <==
\section{Related Work}
% What is offset, skew and drift?
The local notion of time in most sensor-nodes is generated by the oscillator, it provides clock ticks. The literature differentiate three different terms when discussing the non-ideal behaviour of clocks: \textit{Offset} which is the delay between two clocks, when this value is zero, both clocks are perfectly synchronized. \textit{Skew} is the difference between the frequencies of the clocks. \textit{Drift} refers to small variations on the skew, usually as consequence of environmental changes such as Temperature \cite{basics}.    


% How to compensate for offset
    % Why not GPS 
Several papers presented methods to eliminate the clock offset in large-scale networks, passively by using reference signals \cite{airsync} or actively by propagating synchronization-signals over the network \cite{PulseSync}. However, these methods fail to meet the strict synchronization requirements of distributed networks. Currently, GPS synchronization is a widely adopted method for providing accurate synchronization over large distances. Nevertheless, GPS receivers add a non-negligible cost to each node and are prone to spoofing \cite{spoofing}.



% How to compensate for skew and drift
State-of-the-art methods focusing on the compensation of the clock skew and drift are usually conducted for wireless sensor networks with limited RF-capabilities. While some works consider compensation methods based on linear programming and multi-cast \cite{linearprogramming}, most research reports are centered around temperature-assisted methods \cite{linearprogramming,Temp_assisted,Temperature}. This arises from the strong correlation between the working-temperature and the oscillator-frequency. 

Obtaining a good temperature-frequency model requires accurate measurements of the oscillator frequency, which can be challenging to obtain. To this end, some research considers a static model by which the temperature-frequency model is approximated using a second order or third order polynomial \cite{Temp_assisted}. The weights for the second and third order polynomial are estimated using a priory measurements. More recent work focuses on a dynamic model based on lookup-tables and interpolation between known temperature-frequency pairs\cite{nB-iot}. However, most research in this domain targets low-end oscillators which have a more outspoken temperature-frequency correlation compared to the high-end oscillators considered in this work. The required accuracy of the models fail to meet the required accuracy considered in this work. To the best of the authors’ knowledge, LSTM and online-LSTM have not been considered for modeling the temperature-frequency behavior the oscillator. 

%\sofie{State of the art on the use of other signals than GPS, e.g., LTE or ADS-B or....?}

%% How do they estimate the ppm in state of the art? 

==> background.tex <==
\section{Background}
\subsection{SDR; PlutoSDR}
In this research the PlutoSDR is used. This is a mid-tier software defined radio. What makes the PlutoSDR a good candidate is the high-tier RF chip (ad9361) that is used. 
The Pluto has a bad oscillator and therefore we opt to replace the oscillator with a more accurate one. On the internet there are sufficient tutorials that describe how to do this. In the recent versions of the Pluto, there is an external clock input which can be easily connected and used.
Instead of replacing the XO, we added an external reference clock. This external reference clock is the LeoBodnard gps mini reference clock.
When using this device without connecting the gps antenna, the device acts as an higher end oscillator with an accuracy of 0.5 ppm. which is way lower compared. 

\subsection{Clockoffset, skew and drift}
Here I should write about the general concepts like clock drift en skew. providing 


test grammerly  but with a 

==> experimental_setup.tex <==
\subsection{Experimental setup}
The SDR chosen for the experimental setup is the Pluto-SDR produced by Analog Devices \hazem{[REF]}. This SDR is typically targeted at students, engineers and enthusiasts to introduce them to software-defined radios \hazem{no need to say this}. Just say it's a low-cost one used in academia or for educational purposes.. This SDR's relatively low cost and powerful RF-front-end make it an appealing candidate for spectrum sensing networks. However, the SDR is not usable as a sensor out of the box. Since it is considered a learning module, the default XO is a low-end XO \hazem{just say that it has a low-end XO. It's off-the-shelf so no need to motivate why the company made it with low cost XO.} with a ppm of 25 \hazem{this is good to mention}, which is not beneficiary for RF-communication and synchronization purposes. This low-end XO can be replaced, in later versions, starting from rev. c, the Pluto-SDR gained the possibility to connect and select an external reference clock \hazem{again, just say which one we used no need to give details about different versions.}.

\hazem{For the subset of transceivers that has a GPS receiver, we used the Mini ...}The external reference clock selected for this experiment is the Mini Precision GPS Reference Clock, by Leo Bodnar \hazem{add a REF TO THE website OF THE datasheet}. The output frequency of this clock is programmable between 400Hz and 810MHz. When the GPS antenna is connected, the output of the clock is super stable as it is GPS-disciplined. Disconnecting the GPS-antenna results in a high-end programmable oscillator prone to its environment with a maximum ppm of 0.5 between -30 and 85 degrees. 

\hazem{The reader has to wait for two paragraphs to see the setup. I would start with the setup and the fig and then add the details or the explanation for block by block.}
The experimental setup, as can be seen in \ref{fig:setup}, consists of two Pluto-SDRs with a common XO; reference clock. An LTE antenna is connected to one Pluto-SDR; this Pluto-SDR will be considered a node as they occur in the sensor network \hazem{which sensor network? do you mean system model?}. As this work does not consider the offset compensation but skew and drift compensations, only one sensor node is considered for the experiments \hazem{It sounds more negative than positive. It's like you are highlighting what is missing in your paper. You can say. In this work, we focused on the node level, aiming to compensate for any drift and skew that may result from the hardware imperfection.}

\hazem{if you really want you can say we assume that the node of interest are starting from a common clock reference or they have been synced before somehow.}. The second Pluto-SDR is a reference used to evaluate the accuracy of the measurements made by the node \hazem{do you mean that the second one is used to provide the ground truth measurements for our proposed method?}. It is connected to a single-tone generator which produces a single sine on a carrier frequency. As discussed (\hazem{discussed where?}), the GPS antenna connected to the XO, \circled{1} on figure \ref{fig:setup} can be removed. 


\begin{figure}[htbp]
\centerline{\includegraphics[width=0.8\linewidth]{figures/Generic_setup.png}}
\caption{Measurement setup used for experiments}
\label{fig:setup}
\end{figure}




==> figures/training.tex <==
\begin{tikzpicture}

\begin{axis}[
      axis x line=middle,
      axis y line=none,
      height = 0.1\linewidth
      ,
    ]


\addplot [fill=yellow,draw opacity=0, area legend] coordinates {(0,0) (1,1)} \closedcycle;
\addlegendentry{Plot}
\end{axis}
\end{tikzpicture}
